UniCausal: Unified Benchmark and Repository for Causal Text Mining

Current causal text mining datasets vary in objectives, data coverage, and annotation schemes. These inconsistent efforts prevent modeling capabilities and fair comparisons of model performance. Furthermore, few datasets include cause-effect span annotations, which are needed for end-to-end causal relation extraction. To address these issues, we propose UniCausal, a unified benchmark for causal text mining across three tasks: (I) Causal Sequence Classification, (II) Cause-Effect Span Detection and (III) Causal Pair Classification. We consolidated and aligned annotations of six high quality, mainly human-annotated, corpora, resulting in a total of 58,720, 12,144 and 69,165 examples for each task respectively. Since the definition of causality can be subjective, our framework was designed to allow researchers to work on some or all datasets and tasks. To create an initial benchmark, we fine-tuned BERT pre-trained language models to each task, achieving 70.10% Binary F1, 52.42% Macro F1, and 84.68% Binary F1 scores respectively.

==> tabs/AblationResults.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\hline
\multicolumn{1}{l}{\textbf{}} & \multicolumn{4}{c}{Sequence Classification} & \multicolumn{4}{c}{Span Detection} & \multicolumn{4}{c}{Pair Classification} \\ \cline{2-13}
\multicolumn{1}{c}{Model} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} \\\hline
Individual & 71.24 & \textbf{69.52} & \textbf{70.37} & 86.37 & 46.49 & 60.47 & 52.57 & \textbf{78.05} & 87.15 & \textbf{83.22} & \textbf{85.14} & \textbf{93.96} \\
UniCausal ($\alpha=1$) & 70.16 & 65.63 & 67.82 & 85.49 & 49.01 & 61.23 & 54.44 & 77.66 & 88.19 & 75.13 & 81.14 & 92.74 \\
UniCausal ($\alpha=3$) & \textbf{72.66} & 67.37 & 69.92 & \textbf{86.49} & 46.99 & 61.13 & 53.14 & 77.21 & \textbf{89.59} & 75.38 & 81.87 & 93.06 \\
UniCausal ($\alpha=1$), w/ Augment & 72.65 & 61.14 & 66.40 & 85.59 & \textbf{50.34} & \textbf{61.65} & \textbf{55.42} & 77.04 & 88.39 & 74.99 & 81.14 & 92.75
\\\hline
\end{tabular}
}
\caption{Performance for all datasets across three tasks. The top score for each metric per test set is bolded. Scores are reported in percentages (\%). Refer to extended Table \ref{tab:extended_results} in Appendix for performance breakdown by dataset.}\label{tab:ablation_results}
\end{table*}

==> tabs/AtomicResults.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{llllll}\hline
Test Set & Task & P & R & F1 & Acc \\\hline
 ATOMIC & Seq & 100.00 & 77.35 & 87.23 & 77.53 \\
 & Span & 63.73 & 66.72 & 65.19 & 76.53 \\
 & Pair & 100.00 & 75.35 & 85.94 & 75.35 \\\hline
\end{tabular}
}
\caption{Performance metrics for ATOMIC development set. Span Detection task used Macro P/R/F1 scores, while Classification tasks used Binary P/R/F1 scores. ``UniCausal'' model was used, trained concurrently on three tasks for all six datasets, and $\alpha=1$. Scores are reported in percentages (\%).}\label{tab:atomic_results}
\end{table}

==> tabs/ExtendedIndiv.tex <==
\begin{table*}[]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llp{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}}\hline
 &  & \multicolumn{4}{c}{Sequence Classification} & \multicolumn{3}{c}{Span Detection} & \multicolumn{4}{c}{Pair Classification} \\\cline{3-13}
\multicolumn{1}{c}{Test Set} & \multicolumn{1}{c}{Training Set} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} \\\hline

All & All & \textbf{71.13 \textpm0.80} & 69.14 \textpm1.60 & \textbf{70.10 \textpm0.58} & \textbf{86.27 \textpm0.15} & \textbf{46.33 \textpm1.22} & \textbf{60.35 \textpm0.30} & \textbf{52.42 \textpm0.90} & \textbf{85.44 \textpm0.96} & 83.93 \textpm0.44 & \textbf{84.68 \textpm0.27} & \textbf{93.68 \textpm0.16} \\
 & AltLex & 39.77 \textpm3.17*** & 29.03 \textpm7.03*** & 32.93 \textpm3.57*** & 72.90 \textpm2.41*** & 4.29 \textpm0.59*** & 11.21 \textpm1.01*** & 6.20 \textpm0.74*** & 31.68 \textpm9.75*** & 44.64 \textpm23.97* & 31.83 \textpm3.93*** & 61.94 \textpm17.68* \\
 & BECAUSE & 24.74 \textpm1.02*** & \textbf{94.25 \textpm4.07***} & 39.15 \textpm0.99*** & 31.62 \textpm5.62*** & 10.35 \textpm0.29*** & 16.57 \textpm0.59*** & 12.74 \textpm0.35*** & 22.64 \textpm0.70*** & \textbf{93.11 \textpm3.84**} & 36.40 \textpm0.64*** & 32.27 \textpm4.28*** \\
 & CTB & 66.88 \textpm3.05* & 22.66 \textpm4.97*** & 33.49 \textpm5.48*** & 79.30 \textpm0.36*** & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 73.66 \textpm6.50* & 11.83 \textpm3.99*** & 20.17 \textpm5.78*** & 80.78 \textpm0.61*** \\
 & ESL & 28.48 \textpm1.32*** & 65.37 \textpm3.09* & 39.62 \textpm0.89*** & 53.52 \textpm3.61*** & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
 & PDTB & 63.30 \textpm0.66*** & 58.85 \textpm1.29*** & 60.99 \textpm0.76*** & 82.47 \textpm0.26*** & 45.88 \textpm0.65 & 59.92 \textpm0.27** & 51.97 \textpm0.48 & 59.46 \textpm2.15*** & 79.86 \textpm1.46** & 68.13 \textpm0.88*** & 84.45 \textpm0.88*** \\
 & SemEval & 52.00 \textpm2.64*** & 19.44 \textpm1.12*** & 28.25 \textpm0.86*** & 77.02 \textpm0.44*** & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 61.08 \textpm7.17** & 17.23 \textpm2.11*** & 26.66 \textpm1.86*** & 80.37 \textpm0.65***\\\hline
 
AltLex & All & \textbf{50.76 \textpm1.61} & \textbf{63.48 \textpm4.60} & \textbf{56.37 \textpm2.49} & \textbf{71.87 \textpm1.19} & \textbf{27.74 \textpm1.20} & \textbf{42.99 \textpm0.85} & \textbf{33.72 \textpm1.12} & 82.60 \textpm1.99 & \textbf{87.09 \textpm1.53} & \textbf{84.76 \textpm0.66} & \textbf{90.43 \textpm0.55} \\
 & AltLex & 50.58 \textpm3.35 & 53.57 \textpm5.17* & 51.85 \textpm2.53 & 71.52 \textpm1.99 & 16.06 \textpm1.45*** & 32.28 \textpm2.71** & 21.45 \textpm1.87*** & \textbf{88.70 \textpm7.47} & 74.17 \textpm3.40** & 80.57 \textpm2.48* & 89.04 \textpm1.80 \\\hline
 
BECAUSE & All & \textbf{92.32 \textpm1.69} & 70.24 \textpm2.04 & 79.77 \textpm1.68 & 71.37 \textpm2.24 & \textbf{32.51 \textpm2.82} & 44.30 \textpm2.33 & 37.47 \textpm2.57 & \textbf{87.93 \textpm1.73} & 94.78 \textpm1.94 & \textbf{91.21 \textpm1.18} & \textbf{86.00 \textpm1.90} \\
 & BECAUSE & 86.20 \textpm3.31** & \textbf{96.10 \textpm5.06***} & \textbf{90.77 \textpm2.22***} & \textbf{84.31 \textpm3.67***} & 31.15 \textpm5.53 & \textbf{48.17 \textpm5.66} & \textbf{37.79 \textpm5.77} & 83.37 \textpm2.33* & \textbf{97.83 \textpm2.17} & 90.01 \textpm1.95 & 83.33 \textpm3.33 \\\hline
 
CTB & All & 42.37 \textpm2.11 & \textbf{66.19 \textpm4.26} & 51.58 \textpm1.82 & 83.48 \textpm1.21 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 75.66 \textpm3.61 & \textbf{72.50 \textpm6.81} & \textbf{73.94 \textpm4.68} & 95.04 \textpm0.78 \\
 & CTB & \textbf{71.46 \textpm4.90***} & 58.57 \textpm10.59 & \textbf{63.65 \textpm5.55**} & \textbf{91.27 \textpm0.62***} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \textbf{82.18 \textpm7.47} & 67.08 \textpm9.93 & 73.29 \textpm6.14 & \textbf{95.28 \textpm0.96} \\\hline
 
ESL & All & \textbf{76.11 \textpm2.04} & 67.43 \textpm3.45 & 71.45 \textpm1.89 & 73.79 \textpm1.34 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
 & ESL & 75.90 \textpm5.08 & \textbf{87.79 \textpm5.06***} & \textbf{81.21 \textpm2.35***} & \textbf{80.17 \textpm3.00**} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\\hline
 
PDTB & All & 72.59 \textpm0.61 & 66.34 \textpm1.63 & 69.31 \textpm0.70 & 84.63 \textpm0.17 & 47.77 \textpm1.22 & 61.54 \textpm0.29 & 53.78 \textpm0.88 & 84.56 \textpm1.17 & \textbf{82.04 \textpm0.46} & 83.28 \textpm0.36 & 92.43 \textpm0.23 \\
 & PDTB & \textbf{73.54 \textpm0.37*} & \textbf{67.35 \textpm0.90} & \textbf{70.31 \textpm0.56*} & \textbf{85.11 \textpm0.22**} & \textbf{48.89 \textpm0.54} & \textbf{62.92 \textpm0.27***} & \textbf{55.02 \textpm0.38*} & \textbf{86.28 \textpm0.38} & 81.27 \textpm0.36** & \textbf{83.70 \textpm0.34} & \textbf{92.73 \textpm0.15}\\\hline
 
SemEval & All & 73.39 \textpm1.18 & 89.51 \textpm1.59 & 80.64 \textpm0.46 & 94.81 \textpm0.16 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 93.38 \textpm0.88 & 96.10 \textpm0.59 & 94.71 \textpm0.23 & 98.70 \textpm0.07 \\
 & SemEval & \textbf{87.84 \textpm1.49***} & \textbf{91.40 \textpm0.26*} & \textbf{89.58 \textpm0.71***} & \textbf{97.43 \textpm0.20***} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \textbf{93.96 \textpm0.49} & \textbf{95.67 \textpm0.59} & \textbf{94.80 \textpm0.28} & \textbf{98.73 \textpm0.07}\\\hline

\end{tabular}
}
\caption{Performance metrics for different test datasets across the three tasks using Individual models. The top score for each metric per test set is bolded. Tasks that are not applicable to the dataset are indicated by ``-". Scores are reported in percentages (\%). Paired T-test of the models was conducted against setting where all datasets were used for training, with statistical significance indicated by: ***$<0.001$, **$<0.01$, *$<0.05$. The first segment of the table corresponds to Table \ref{tab:indiv_results}.}\label{tab:extended_indiv}
\end{table*}

==> tabs/ExtendedIndiv2.tex <==
\clearpage
% \begin{table*}[]
\begin{landscape}
{\small\tabcolsep=3pt  % hold it local
\begin{longtable}{p{8mm}p{10mm}p{9mm}p{9mm}p{9mm}p{9mm}p{9mm}p{9mm}p{9mm}p{9mm}p{9mm}p{9mm}p{9mm}}\hline
 &  & \multicolumn{4}{c}{(I) Sequence Classification} & \multicolumn{3}{c}{(II) Span Detection} & \multicolumn{4}{c}{(III) Pair Classification} \\\cline{3-13}
\multicolumn{1}{c}{Test Set} & \multicolumn{1}{c}{Training Set} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} \\\hline

All & All & \textbf{71.13 \textpm0.80} & 69.14 \textpm1.60 & \textbf{70.10 \textpm0.58} & \textbf{86.27 \textpm0.15} & \textbf{46.33 \textpm1.22} & \textbf{60.35 \textpm0.30} & \textbf{52.42 \textpm0.90} & \textbf{85.44 \textpm0.96} & 83.93 \textpm0.44 & \textbf{84.68 \textpm0.27} & \textbf{93.68 \textpm0.16} \\
 & AltLex & 39.77 \textpm3.17*** & 29.03 \textpm7.03*** & 32.93 \textpm3.57*** & 72.90 \textpm2.41*** & 4.29 \textpm0.59*** & 11.21 \textpm1.01*** & 6.20 \textpm0.74*** & 31.68 \textpm9.75*** & 44.64 \textpm23.97* & 31.83 \textpm3.93*** & 61.94 \textpm17.68* \\
 & BECAUSE & 24.74 \textpm1.02*** & \textbf{94.25 \textpm4.07***} & 39.15 \textpm0.99*** & 31.62 \textpm5.62*** & 10.35 \textpm0.29*** & 16.57 \textpm0.59*** & 12.74 \textpm0.35*** & 22.64 \textpm0.70*** & \textbf{93.11 \textpm3.84**} & 36.40 \textpm0.64*** & 32.27 \textpm4.28*** \\
 & CTB & 66.88 \textpm3.05* & 22.66 \textpm4.97*** & 33.49 \textpm5.48*** & 79.30 \textpm0.36*** & - & - & - & 73.66 \textpm6.50* & 11.83 \textpm3.99*** & 20.17 \textpm5.78*** & 80.78 \textpm0.61*** \\
 & ESL & 28.48 \textpm1.32*** & 65.37 \textpm3.09* & 39.62 \textpm0.89*** & 53.52 \textpm3.61*** & - & - & - & - & - & - & - \\
 & PDTB & 63.30 \textpm0.66*** & 58.85 \textpm1.29*** & 60.99 \textpm0.76*** & 82.47 \textpm0.26*** & 45.88 \textpm0.65 & 59.92 \textpm0.27** & 51.97 \textpm0.48 & 59.46 \textpm2.15*** & 79.86 \textpm1.46** & 68.13 \textpm0.88*** & 84.45 \textpm0.88*** \\
 & SemEval & 52.00 \textpm2.64*** & 19.44 \textpm1.12*** & 28.25 \textpm0.86*** & 77.02 \textpm0.44*** & - & - & - & 61.08 \textpm7.17** & 17.23 \textpm2.11*** & 26.66 \textpm1.86*** & 80.37 \textpm0.65*** \\
\hline
AltLex & All & \textbf{50.76 \textpm1.61} & 63.48 \textpm4.60 & \textbf{56.37 \textpm2.49} & 71.87 \textpm1.19 & \textbf{27.74 \textpm1.20} & \textbf{42.99 \textpm0.85} & \textbf{33.72 \textpm1.12} & 82.60 \textpm1.99 & 87.09 \textpm1.53 & \textbf{84.76 \textpm0.66} & \textbf{90.43 \textpm0.55} \\
 & AltLex & 50.58 \textpm3.35 & 53.57 \textpm5.17* & 51.85 \textpm2.53 & 71.52 \textpm1.99 & 16.06 \textpm1.45*** & 32.28 \textpm2.71** & 21.45 \textpm1.87*** & \textbf{88.70 \textpm7.47} & 74.17 \textpm3.40** & 80.57 \textpm2.48* & 89.04 \textpm1.80 \\
 & BECAUSE & 31.69 \textpm1.90*** & 91.83 \textpm5.45*** & 47.02 \textpm1.52** & 40.40 \textpm7.17*** & 5.65 \textpm1.89*** & 10.71 \textpm2.42*** & 7.38 \textpm2.19*** & 32.14 \textpm1.18*** & \textbf{94.80 \textpm1.98***} & 47.99 \textpm1.33*** & 37.21 \textpm3.34*** \\
 & CTB & 63.35 \textpm3.23** & 51.65 \textpm13.15 & 55.91 \textpm7.63 & \textbf{77.36 \textpm1.13**} & - & - & - & 84.28 \textpm18.29 & 12.60 \textpm13.35*** & 19.16 \textpm15.64*** & 71.83 \textpm1.64*** \\
 & ESL & 30.83 \textpm1.37*** & \textbf{93.57 \textpm6.81**} & 46.29 \textpm1.15** & 37.66 \textpm5.74*** & - & - & - & - & - & - & - \\
 & PDTB & 48.02 \textpm2.10 & 49.91 \textpm2.00** & 48.94 \textpm1.88** & 70.12 \textpm1.28 & 5.36 \textpm0.81*** & 9.06 \textpm1.11*** & 6.73 \textpm0.94*** & 26.73 \textpm0.89*** & 82.20 \textpm4.26 & 40.34 \textpm1.52*** & 25.82 \textpm1.14*** \\
 & SemEval & 55.23 \textpm2.44* & 19.65 \textpm1.58*** & 28.95 \textpm1.74*** & 72.37 \textpm0.48 & - & - & - & 72.07 \textpm2.90*** & 25.35 \textpm6.21*** & 37.07 \textpm6.58*** & 74.13 \textpm0.91*** \\
\hline
BEC- AUSE & All & 92.32 \textpm1.69 & 70.24 \textpm2.04 & 79.77 \textpm1.68 & 71.37 \textpm2.24 & \textbf{32.51 \textpm2.82} & 44.30 \textpm2.33 & 37.47 \textpm2.57 & \textbf{87.93 \textpm1.73} & 94.78 \textpm1.94 & \textbf{91.21 \textpm1.18} & \textbf{86.00 \textpm1.90} \\
 & AltLex & 98.67 \textpm2.98* & 22.93 \textpm8.73*** & 36.47 \textpm11.18*** & 37.65 \textpm6.41*** & 8.30 \textpm1.40*** & 18.92 \textpm2.10*** & 11.51 \textpm1.63*** & 80.49 \textpm7.19 & 37.83 \textpm21.33** & 48.44 \textpm20.00** & 45.00 \textpm12.19** \\
 & BECAUSE & 86.20 \textpm3.31** & 96.10 \textpm5.06*** & \textbf{90.77 \textpm2.22***} & \textbf{84.31 \textpm3.67***} & 31.15 \textpm5.53 & \textbf{48.17 \textpm5.66} & \textbf{37.79 \textpm5.77} & 83.37 \textpm2.33* & \textbf{97.83 \textpm2.17} & 90.01 \textpm1.95 & 83.33 \textpm3.33 \\
 & CTB & \textbf{97.87 \textpm2.94*} & 38.54 \textpm8.86** & 54.73 \textpm9.40** & 49.80 \textpm6.59** & - & - & - & 84.90 \textpm11.92 & 13.04 \textpm7.37*** & 22.00 \textpm10.92*** & 31.67 \textpm4.86*** \\
 & ESL & 83.42 \textpm1.02*** & \textbf{98.05 \textpm2.67***} & 90.12 \textpm1.05*** & 82.75 \textpm1.64** & - & - & - & - & - & - & - \\
 & PDTB & 89.33 \textpm1.57* & 57.07 \textpm2.78** & 69.61 \textpm2.16** & 60.00 \textpm2.24** & 32.50 \textpm2.77 & 40.00 \textpm1.92 & 35.84 \textpm2.42 & 77.99 \textpm1.47*** & 87.83 \textpm3.95** & 82.59 \textpm2.17*** & 71.67 \textpm3.12*** \\
 & SemEval & 100.00 \textpm0.00*** & 9.27 \textpm2.04*** & 16.91 \textpm3.40*** & 27.06 \textpm1.64*** & - & - & - & 98.18 \textpm4.07** & 15.22 \textpm7.37*** & 25.70 \textpm11.46*** & 34.67 \textpm5.32*** \\
\hline
CTB & All & 42.37 \textpm2.11 & 66.19 \textpm4.26 & 51.58 \textpm1.82 & 83.48 \textpm1.21 & - & - & - & 75.66 \textpm3.61 & 72.50 \textpm6.81 & \textbf{73.94 \textpm4.68} & 95.04 \textpm0.78 \\
 & AltLex & 40.43 \textpm6.72 & 39.05 \textpm13.94* & 38.21 \textpm6.20* & 83.80 \textpm2.37 & - & - & - & 20.48 \textpm9.28*** & 35.42 \textpm24.87* & 20.06 \textpm7.14*** & 74.84 \textpm14.26* \\
 & BECAUSE & 14.45 \textpm0.92*** & \textbf{98.10 \textpm1.99***} & 25.17 \textpm1.34*** & 22.15 \textpm7.02*** & - & - & - & 13.42 \textpm0.99*** & \textbf{97.50 \textpm0.93**} & 23.58 \textpm1.52*** & 38.09 \textpm5.14*** \\
 & CTB & \textbf{71.46 \textpm4.90***} & 58.57 \textpm10.59 & \textbf{63.65 \textpm5.55**} & \textbf{91.27 \textpm0.62***} & - & - & - & \textbf{82.18 \textpm7.47} & 67.08 \textpm9.93 & 73.29 \textpm6.14 & \textbf{95.28 \textpm0.96} \\
 & ESL & 18.48 \textpm0.91*** & 93.33 \textpm4.58*** & 30.84 \textpm1.35*** & 44.30 \textpm3.50*** & - & - & - & - & - & - & - \\
 & PDTB & 33.36 \textpm1.77** & 48.57 \textpm2.71*** & 39.54 \textpm1.88*** & 80.25 \textpm0.86* & - & - & - & 16.97 \textpm1.26*** & 64.17 \textpm13.13 & 26.74 \textpm2.42*** & 65.98 \textpm3.86*** \\
 & SemEval & 49.19 \textpm4.13* & 31.90 \textpm4.33*** & 38.51 \textpm3.44** & 86.52 \textpm0.76* & - & - & - & 46.94 \textpm3.96*** & 55.42 \textpm3.49** & 50.63 \textpm1.74*** & 89.43 \textpm1.09*** \\
\hline
ESL & All & 76.11 \textpm2.04 & 67.43 \textpm3.45 & 71.45 \textpm1.89 & 73.79 \textpm1.34 & - & - & - & - & - & - & - \\
 & AltLex & 45.40 \textpm3.38*** & 65.84 \textpm18.33 & 53.30 \textpm8.37** & 45.60 \textpm3.77*** & - & - & - & - & - & - & - \\
 & BECAUSE & 48.17 \textpm1.05*** & \textbf{93.27 \textpm5.89**} & 63.49 \textpm1.94** & 47.84 \textpm1.95*** & - & - & - & - & - & - & - \\
 & CTB & \textbf{92.10 \textpm7.32*} & 21.42 \textpm12.01** & 33.26 \textpm15.44** & 60.69 \textpm4.70** & - & - & - & - & - & - & - \\
 & ESL & 75.90 \textpm5.08 & 87.79 \textpm5.06*** & \textbf{81.21 \textpm2.35***} & \textbf{80.17 \textpm3.00**} & - & - & - & - & - & - & - \\
 & PDTB & 68.44 \textpm8.81 & 27.26 \textpm3.39*** & 38.71 \textpm3.15*** & 58.10 \textpm2.16*** & - & - & - & - & - & - & - \\
 & SemEval & 42.91 \textpm1.95*** & 49.56 \textpm5.70*** & 45.95 \textpm3.50*** & 43.45 \textpm1.86*** & - & - & - & - & - & - & - \\
\hline
PDTB & All & 72.59 \textpm0.61 & 66.34 \textpm1.63 & 69.31 \textpm0.70 & 84.63 \textpm0.17 & \textbf{47.77 \textpm1.22} & \textbf{61.54 \textpm0.29} & \textbf{53.78 \textpm0.88} & 84.56 \textpm1.17 & 82.04 \textpm0.46 & 83.28 \textpm0.36 & 92.43 \textpm0.23 \\
 & AltLex & 34.38 \textpm2.46*** & 17.92 \textpm6.86*** & 22.91 \textpm5.79*** & 69.49 \textpm1.84*** & 3.77 \textpm0.60*** & 9.97 \textpm1.04*** & 5.47 \textpm0.76*** & 24.08 \textpm3.84*** & 39.15 \textpm28.09* & 25.11 \textpm8.75*** & 54.18 \textpm20.53* \\
 & BECAUSE & 27.49 \textpm0.92*** & \textbf{93.87 \textpm4.32***} & 42.49 \textpm0.68*** & 33.39 \textpm4.95*** & 10.28 \textpm0.28*** & 16.28 \textpm0.58*** & 12.60 \textpm0.34*** & 24.24 \textpm0.52*** & \textbf{92.47 \textpm4.46**} & 38.39 \textpm0.37*** & 31.81 \textpm3.78*** \\
 & CTB & 66.42 \textpm3.44** & 16.30 \textpm3.22*** & 25.97 \textpm3.73*** & 75.87 \textpm0.09*** & - & - & - & 83.73 \textpm8.27 & 3.77 \textpm3.43*** & 7.02 \textpm6.06*** & 77.74 \textpm0.65*** \\
 & ESL & 33.97 \textpm1.57*** & 57.18 \textpm3.51** & 42.55 \textpm1.25*** & 59.58 \textpm2.58*** & - & - & - & - & - & - & - \\
 & PDTB & \textbf{73.54 \textpm0.37*} & 67.35 \textpm0.90 & \textbf{70.31 \textpm0.56*} & \textbf{85.11 \textpm0.22**} & 48.89 \textpm0.54 & 62.92 \textpm0.27*** & 55.02 \textpm0.38* & \textbf{86.28 \textpm0.38} & 81.27 \textpm0.36** & \textbf{83.70 \textpm0.34} & \textbf{92.73 \textpm0.15} \\
 & SemEval & 27.47 \textpm0.84*** & 6.24 \textpm1.24*** & 10.11 \textpm1.61*** & 71.13 \textpm0.65*** & - & - & - & 29.32 \textpm3.92*** & 4.80 \textpm2.19*** & 8.08 \textpm3.20*** & 75.46 \textpm0.86*** \\
\hline
Sem- Eval & All & 73.39 \textpm1.18 & 89.51 \textpm1.59 & 80.64 \textpm0.46 & 94.81 \textpm0.16 & - & - & - & 93.38 \textpm0.88 & \textbf{96.10 \textpm0.59} & 94.71 \textpm0.23 & 98.70 \textpm0.07 \\
 & AltLex & 44.85 \textpm9.44** & 76.89 \textpm5.62* & 55.83 \textpm6.68*** & 84.68 \textpm5.49* & - & - & - & 50.83 \textpm19.73** & 73.90 \textpm5.42** & 57.72 \textpm14.52** & 84.33 \textpm12.18 \\
 & BECAUSE & 13.52 \textpm1.28*** & \textbf{97.13 \textpm2.20***} & 23.71 \textpm1.93*** & 23.91 \textpm8.67*** & - & - & - & 14.56 \textpm1.40*** & 95.61 \textpm2.53 & 25.23 \textpm2.02*** & 31.00 \textpm8.75*** \\
 & CTB & 63.55 \textpm4.28** & 46.16 \textpm16.86** & 51.76 \textpm13.85** & 90.27 \textpm1.03*** & - & - & - & 68.73 \textpm7.25** & 59.63 \textpm6.21*** & 63.69 \textpm5.65*** & 91.79 \textpm1.36*** \\
 & ESL & 15.33 \textpm1.93*** & 91.40 \textpm7.82 & 26.15 \textpm2.62*** & 36.57 \textpm12.82*** & - & - & - &  &  &  &  \\
 & PDTB & 18.60 \textpm2.29*** & 21.16 \textpm4.87*** & 19.75 \textpm3.35*** & 79.40 \textpm0.51*** & - & - & - & 22.25 \textpm1.33*** & 70.24 \textpm9.89** & 33.64 \textpm1.76*** & 66.60 \textpm4.06*** \\
 & SemEval & \textbf{87.84 \textpm1.49***} & 91.40 \textpm0.26* & \textbf{89.58 \textpm0.71***} & \textbf{97.43 \textpm0.20***} & - & - & - & \textbf{93.96 \textpm0.49} & 95.67 \textpm0.59 & \textbf{94.80 \textpm0.28} & \textbf{98.73 \textpm0.07}\\\hline
\caption{Performance metrics for different test datasets across the three tasks using Individual models. The top score for each metric per test set is bolded. Tasks that are not applicable to the dataset are indicated by ``-". Scores are reported in percentages (\%). Paired T-test of the models was conducted against setting where all datasets were used for training, with statistical significance indicated by: ***$<0.001$, **$<0.01$, *$<0.05$. For each test set, the first row (i.e. when training set is ``All") is consolidated and corresponds to Table \ref{tab:extended_results2}. The F1 scores of this table also corresponds to the values consolidated in Table \ref{tab:matrix}.}
\label{tab:extended_indiv2}
\end{longtable}
}% end
\end{landscape}
\clearpage

==> tabs/ExtendedResults.tex <==
\begin{table*}[]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{lp{30mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}}\hline
 &  & \multicolumn{4}{c}{Sequence Classification} & \multicolumn{3}{c}{Span Detection} & \multicolumn{4}{c}{Pair Classification} \\\cline{3-13}
\multicolumn{1}{c}{Test Set} & \multicolumn{1}{c}{Model} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} \\\hline

All & Individual & 71.13 \textpm0.80 & \textbf{69.14 \textpm1.60} & \textbf{70.10 \textpm0.58} & \textbf{86.27 \textpm0.15} & 46.33 \textpm1.22 & 60.35 \textpm0.30 & 52.42 \textpm0.90 & 85.44 \textpm0.96 & \textbf{83.93 \textpm0.44} & \textbf{84.68 \textpm0.27} & \textbf{93.68 \textpm0.16} \\
 & UniCausal ($\alpha=1$) & 70.88 \textpm0.60 & 64.67 \textpm0.70** & 67.63 \textpm0.24** & 85.58 \textpm0.12** & 52.21 \textpm0.64*** & 60.86 \textpm0.55 & 56.21 \textpm0.60*** & 88.47 \textpm0.52** & 75.55 \textpm0.58*** & 81.50 \textpm0.30*** & 92.87 \textpm0.10** \\
 & UniCausal ($\alpha=3$) & 72.12 \textpm0.66 & 66.80 \textpm1.10** & 69.35 \textpm0.47** & 86.25 \textpm0.16 & 49.44 \textpm1.90** & 60.10 \textpm0.64 & 54.24 \textpm1.41* & 88.77 \textpm0.54*** & 76.51 \textpm1.24*** & 82.18 \textpm0.53*** & 93.10 \textpm0.14** \\
 & UniCausal ($\alpha=1$), w/ Augment & \textbf{72.39 \textpm0.77} & 61.39 \textpm0.79*** & 66.43 \textpm0.36*** & 85.55 \textpm0.17** & \textbf{52.36 \textpm0.99**} & \textbf{61.26 \textpm0.55} & \textbf{56.46 \textpm0.70**} & \textbf{88.79 \textpm0.80**} & 74.32 \textpm1.16*** & 80.91 \textpm0.51*** & 92.71 \textpm0.15*** \\\hline
 
AltLex & Individual & 50.76 \textpm1.61 & \textbf{63.48 \textpm4.60} & 56.37 \textpm2.49 & 71.87 \textpm1.19 & 27.74 \textpm1.20 & \textbf{42.99 \textpm0.85} & 33.72 \textpm1.12 & 82.60 \textpm1.99 & \textbf{87.09 \textpm1.53} & \textbf{84.76 \textpm0.66} & \textbf{90.43 \textpm0.55} \\
 & UniCausal ($\alpha=1$) & 56.98 \textpm2.00** & 61.91 \textpm2.78 & \textbf{59.32 \textpm2.06} & \textbf{75.66 \textpm1.20**} & \textbf{29.78 \textpm1.32} & 39.21 \textpm1.23* & 33.85 \textpm1.29 & 83.50 \textpm3.18 & 74.33 \textpm4.19** & 78.57 \textpm2.61* & 87.64 \textpm1.41* \\
 & UniCausal ($\alpha=3$) & 55.24 \textpm1.73* & 63.13 \textpm3.72 & 58.90 \textpm2.38 & 74.76 \textpm1.13* & 25.70 \textpm2.76* & 38.43 \textpm0.72*** & 30.72 \textpm1.98** & 85.21 \textpm2.26* & 78.43 \textpm4.11** & 81.60 \textpm2.03* & 89.23 \textpm1.01 \\
 & UniCausal ($\alpha=1$), w/ Augment & \textbf{57.64 \textpm2.43*} & 53.22 \textpm3.22* & 55.31 \textpm2.58 & 75.36 \textpm1.29* & 29.33 \textpm0.91 & 40.47 \textpm1.63 & \textbf{34.01 \textpm1.18} & \textbf{88.43 \textpm1.74*} & 78.11 \textpm4.87* & 82.89 \textpm2.96 & 90.19 \textpm1.48 \\\hline
 
BECAUSE & Individual & \textbf{92.32 \textpm1.69} & \textbf{70.24 \textpm2.04} & \textbf{79.77 \textpm1.68} & \textbf{71.37 \textpm2.24} & 32.51 \textpm2.82 & 44.30 \textpm2.33 & 37.47 \textpm2.57 & 87.93 \textpm1.73 & \textbf{94.78 \textpm1.94} & \textbf{91.21 \textpm1.18} & \textbf{86.00 \textpm1.90} \\
 & UniCausal ($\alpha=1$) & 90.14 \textpm1.58 & 62.44 \textpm2.78* & 73.75 \textpm2.23* & 64.31 \textpm2.56* & \textbf{38.80 \textpm3.15*} & \textbf{47.53 \textpm2.57} & \textbf{42.70 \textpm2.78*} & 91.45 \textpm1.40* & 83.91 \textpm4.24** & 87.49 \textpm2.76* & 81.67 \textpm3.73* \\
 & UniCausal ($\alpha=3$) & 90.78 \textpm2.42 & 63.41 \textpm6.90 & 74.56 \textpm5.51 & 65.49 \textpm6.29 & 37.98 \textpm5.50* & 44.95 \textpm3.17 & 41.02 \textpm4.18 & 91.75 \textpm2.04** & 86.96 \textpm3.44* & 89.27 \textpm2.43 & 84.00 \textpm3.46 \\
 & UniCausal ($\alpha=1$), w/ Augment & 89.89 \textpm2.39 & 52.20 \textpm3.70** & 66.00 \textpm3.36** & 56.86 \textpm3.40** & 38.74 \textpm4.05 & 45.38 \textpm3.35 & 41.75 \textpm3.54 & \textbf{91.99 \textpm1.09*} & 80.00 \textpm5.41** & 85.51 \textpm3.36* & 79.33 \textpm4.18* \\\hline
 
CTB & Individual & 42.37 \textpm2.11 & \textbf{66.19 \textpm4.26} & 51.58 \textpm1.82 & 83.48 \textpm1.21 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 75.66 \textpm3.61 & \textbf{72.50 \textpm6.81} & \textbf{73.94 \textpm4.68} & \textbf{95.04 \textpm0.78} \\
 & UniCausal ($\alpha=1$) & 43.32 \textpm1.93 & 61.43 \textpm3.10 & 50.79 \textpm2.06 & 84.18 \textpm0.81 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 80.11 \textpm4.92 & 37.92 \textpm2.72*** & 51.38 \textpm2.59*** & 93.01 \textpm0.34** \\
 & UniCausal ($\alpha=3$) & \textbf{44.96 \textpm2.21} & 61.90 \textpm2.92 & \textbf{52.01 \textpm1.26} & \textbf{84.81 \textpm0.92} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \textbf{82.68 \textpm6.63} & 43.33 \textpm6.14*** & 56.48 \textpm4.75*** & 93.54 \textpm0.49** \\
 & UniCausal ($\alpha=1$), w/ Augment & 39.68 \textpm4.10 & 47.62 \textpm3.76** & 43.23 \textpm3.55* & 83.35 \textpm1.37 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 80.27 \textpm12.32 & 26.67 \textpm5.19*** & 39.51 \textpm4.84*** & 92.11 \textpm0.36** \\\hline
 
ESL & Individual & 76.11 \textpm2.04 & \textbf{67.43 \textpm3.45} & \textbf{71.45 \textpm1.89} & 73.79 \textpm1.34 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
 & UniCausal ($\alpha=1$) & 76.68 \textpm3.34 & 61.06 \textpm3.13* & 67.90 \textpm1.77* & 71.90 \textpm1.54 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
 & UniCausal ($\alpha=3$) & \textbf{78.87 \textpm2.60} & 63.89 \textpm3.28 & 70.55 \textpm2.40 & \textbf{74.05 \textpm1.86} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
 & UniCausal ($\alpha=1$), w/ Augment & 76.45 \textpm2.99 & 62.65 \textpm3.33 & 68.78 \textpm1.77 & 72.33 \textpm1.41 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\\hline
 
PDTB & Individual & 72.59 \textpm0.61 & \textbf{66.34 \textpm1.63} & \textbf{69.31 \textpm0.70} & 84.63 \textpm0.17 & 47.77 \textpm1.22 & 61.54 \textpm0.29 & 53.78 \textpm0.88 & 84.56 \textpm1.17 & \textbf{82.04 \textpm0.46} & \textbf{83.28 \textpm0.36} & \textbf{92.43 \textpm0.23} \\
 & UniCausal ($\alpha=1$) & 72.92 \textpm0.96 & 61.45 \textpm1.08** & 66.68 \textpm0.27** & 83.93 \textpm0.14** & 53.83 \textpm0.72*** & 62.25 \textpm0.57* & 57.74 \textpm0.65*** & 87.99 \textpm0.56** & 74.04 \textpm0.73*** & 80.41 \textpm0.43*** & 91.71 \textpm0.16* \\
 & UniCausal ($\alpha=3$) & 73.98 \textpm0.78* & 63.86 \textpm1.28** & 68.54 \textpm0.69* & \textbf{84.66 \textpm0.26} & 51.23 \textpm1.64** & 61.52 \textpm0.69 & 55.90 \textpm1.26** & \textbf{88.19 \textpm0.36***} & 74.64 \textpm1.15*** & 80.84 \textpm0.57** & 91.88 \textpm0.18* \\
 & UniCausal ($\alpha=1$), w/ Augment & \textbf{74.01 \textpm0.96} & 58.14 \textpm1.06*** & 65.11 \textpm0.52*** & 83.69 \textpm0.21*** & \textbf{54.06 \textpm1.02**} & \textbf{62.65 \textpm0.56*} & \textbf{58.04 \textpm0.70**} & \textbf{88.19 \textpm0.87**} & 72.71 \textpm1.32*** & 79.70 \textpm0.66*** & 91.49 \textpm0.22*** \\\hline
 
SemEval & Individual & \textbf{73.39 \textpm1.18} & \textbf{89.51 \textpm1.59} & \textbf{80.64 \textpm0.46} & \textbf{94.81 \textpm0.16} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 93.38 \textpm0.88 & \textbf{96.10 \textpm0.59} & \textbf{94.71 \textpm0.23} & \textbf{98.70 \textpm0.07} \\
 & UniCausal ($\alpha=1$) & 68.10 \textpm1.49*** & 87.74 \textpm1.45 & 76.67 \textpm0.93*** & 93.55 \textpm0.32*** & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 93.42 \textpm0.39 & 90.91 \textpm0.59*** & 92.15 \textpm0.48** & 98.13 \textpm0.11** \\
 & UniCausal ($\alpha=3$) & 70.49 \textpm0.88*** & 88.54 \textpm1.34 & 78.49 \textpm0.93** & 94.14 \textpm0.25*** & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \textbf{93.71 \textpm1.36} & 92.26 \textpm1.19** & 92.97 \textpm0.60** & 98.31 \textpm0.15* \\
 & UniCausal ($\alpha=1$), w/ Augment & 71.99 \textpm1.08 & 87.07 \textpm1.41* & 78.81 \textpm0.79* & 94.34 \textpm0.22* & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 92.57 \textpm1.31 & 90.30 \textpm0.66*** & 91.42 \textpm0.84*** & 97.95 \textpm0.21***\\\hline
 
\end{tabular}
}
\caption{Performance metrics for different test sets across the three tasks. ``Individual'' refers to baseline models trained on a single task, whereas ``UniCausal" refers to our proposed model that concurrently trains on three tasks and $\alpha=1$. All models were trained on all six datasets. The top score for each metric per test set is bolded. Tasks that are not applicable to the dataset are indicated by ``-". Scores are reported in percentages (\%). Paired T-test of the UniCausal models was conducted against the Individual model per Test Set, with statistical significance indicated by: ***$<0.001$, **$<0.01$, *$<0.05$. The first segment of the table corresponds to Table \ref{tab:main_results}.}\label{tab:extended_results}
\end{table*}

==> tabs/IndivResults.tex <==
\begin{table*}[]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{p{20mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}}\hline
 & \multicolumn{4}{c}{Sequence Classification} & \multicolumn{3}{c}{Span Detection} & \multicolumn{4}{c}{Pair Classification} \\\cline{2-12}
\multicolumn{1}{c}{Training Set} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} \\\hline

All & \textbf{71.13 \textpm0.80} & 69.14 \textpm1.60 & \textbf{70.10 \textpm0.58} & \textbf{86.27 \textpm0.15} & \textbf{46.33 \textpm1.22} & \textbf{60.35 \textpm0.30} & \textbf{52.42 \textpm0.90} & \textbf{85.44 \textpm0.96} & 83.93 \textpm0.44 & \textbf{84.68 \textpm0.27} & \textbf{93.68 \textpm0.16} \\\hline
AltLex & 39.77 \textpm3.17*** & 29.03 \textpm7.03*** & 32.93 \textpm3.57*** & 72.90 \textpm2.41*** & 4.29 \textpm0.59*** & 11.21 \textpm1.01*** & 6.20 \textpm0.74*** & 31.68 \textpm9.75*** & 44.64 \textpm23.97* & 31.83 \textpm3.93*** & 61.94 \textpm17.68* \\
BECAUSE & 24.74 \textpm1.02*** & \textbf{94.25 \textpm4.07***} & 39.15 \textpm0.99*** & 31.62 \textpm5.62*** & 10.35 \textpm0.29*** & 16.57 \textpm0.59*** & 12.74 \textpm0.35*** & 22.64 \textpm0.70*** & \textbf{93.11 \textpm3.84**} & 36.40 \textpm0.64*** & 32.27 \textpm4.28*** \\
CTB & 66.88 \textpm3.05* & 22.66 \textpm4.97*** & 33.49 \textpm5.48*** & 79.30 \textpm0.36*** & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 73.66 \textpm6.50* & 11.83 \textpm3.99*** & 20.17 \textpm5.78*** & 80.78 \textpm0.61*** \\
ESL & 28.48 \textpm1.32*** & 65.37 \textpm3.09* & 39.62 \textpm0.89*** & 53.52 \textpm3.61*** & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
PDTB & 63.30 \textpm0.66*** & 58.85 \textpm1.29*** & 60.99 \textpm0.76*** & 82.47 \textpm0.26*** & 45.88 \textpm0.65 & 59.92 \textpm0.27** & 51.97 \textpm0.48 & 59.46 \textpm2.15*** & 79.86 \textpm1.46** & 68.13 \textpm0.88*** & 84.45 \textpm0.88*** \\
SemEval & 52.00 \textpm2.64*** & 19.44 \textpm1.12*** & 28.25 \textpm0.86*** & 77.02 \textpm0.44*** & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 61.08 \textpm7.17** & 17.23 \textpm2.11*** & 26.66 \textpm1.86*** & 80.37 \textpm0.65***\\\hline
 
\end{tabular}
}
\caption{Performance metrics for on all six datasets when using different training sets. The Individual models were used for each of the three tasks. The top score per column is bolded. Tasks that are not applicable to the dataset are indicated by ``-". Scores are reported in percentages (\%). Paired T-test of the models was conducted against the first row, where all datasets were used for training, with statistical significance indicated by: ***$<0.001$, **$<0.01$, *$<0.05$. Refer to extended Table \ref{tab:extended_indiv} in Appendix for performance breakdown by dataset.}\label{tab:indiv_results}
\end{table*}

==> tabs/MainResults.tex <==
\begin{table*}[]
\centering
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{p{30mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}p{10mm}}\hline
 & \multicolumn{4}{c}{Sequence Classification} & \multicolumn{3}{c}{Span Detection} & \multicolumn{4}{c}{Pair Classification} \\\cline{2-12}
\multicolumn{1}{c}{Model} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Acc} \\\hline
Individual & 71.13 \textpm0.80 & \textbf{69.14 \textpm1.60} & \textbf{70.10 \textpm0.58} & \textbf{86.27 \textpm0.15} & 46.33 \textpm1.22 & 60.35 \textpm0.30 & 52.42 \textpm0.90 & 85.44 \textpm0.96 & \textbf{83.93 \textpm0.44} & \textbf{84.68 \textpm0.27} & \textbf{93.68 \textpm0.16} \\
UniCausal ($\alpha=1$) & 70.88 \textpm0.60 & 64.67 \textpm0.70** & 67.63 \textpm0.24** & 85.58 \textpm0.12** & 52.21 \textpm0.64*** & 60.86 \textpm0.55 & 56.21 \textpm0.60*** & 88.47 \textpm0.52** & 75.55 \textpm0.58*** & 81.50 \textpm0.30*** & 92.87 \textpm0.10** \\
UniCausal ($\alpha=3$) & 72.12 \textpm0.66 & 66.80 \textpm1.10** & 69.35 \textpm0.47** & 86.25 \textpm0.16 & 49.44 \textpm1.90** & 60.10 \textpm0.64 & 54.24 \textpm1.41* & 88.77 \textpm0.54*** & 76.51 \textpm1.24*** & 82.18 \textpm0.53*** & 93.10 \textpm0.14** \\
UniCausal ($\alpha=1$), w/ Augment & \textbf{72.39 \textpm0.77} & 61.39 \textpm0.79*** & 66.43 \textpm0.36*** & 85.55 \textpm0.17** & \textbf{52.36 \textpm0.99**} & \textbf{61.26 \textpm0.55} & \textbf{56.46 \textpm0.70**} & \textbf{88.79 \textpm0.80**} & 74.32 \textpm1.16*** & 80.91 \textpm0.51*** & 92.71 \textpm0.15*** \\\hline
\end{tabular}
}
\caption{Performance for all datasets across three tasks. The top score for each metric per test set is bolded. Scores are reported in percentages (\%). Paired T-test of the models was conducted against the Individual model, with statistical significance indicated by: ***$<0.001$, **$<0.01$, *$<0.05$. Refer to extended Table \ref{tab:extended_results} in Appendix for performance breakdown by dataset. }\label{tab:main_results}
\end{table*}

==> tabs/RawData.tex <==
\begin{table*}[]
\centering
\begin{tabular}{l|llll|l}\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Corpus}} & \multicolumn{4}{c}{Number of Sentences} & \multicolumn{1}{|c}{\multirow{2}{*}{Total}} \\\cline{2-5}
\multicolumn{1}{c|}{} & 1 & 2 & 3 & \textgreater{}3 & \multicolumn{1}{c}{} \\\hline
AltLex & 1,027 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} & 1,027 \\
BECAUSE & 1,245 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} & 1,245 \\
CTB & 3,043 & 578 & 188 & 390 & 4,199 \\
ESL & 7,140 & 6,487 & 5,754 & 19,753 & 39,134 \\
PDTB & 28,088 & 22,945 & 1,468 & 1,175 & 53,676 \\
SemEval & 10,717 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} & 10,717 \\\hline
Total & 51,260 & 30,010 & 7,410 & 21,318 & 109,998\\\hline
\end{tabular}
\caption{Sizes of raw datasets by sentence length.}\label{tab:raw_data}
\end{table*}

==> tabs/RawData2.tex <==
\begin{table*}[]
\centering
\begin{tabular}{l|l|lll|l}\hline
\multirow{2}{*}{Corpus} & \multirow{2}{*}{Split} & \multicolumn{3}{c|}{Number of Sentences} & \multirow{2}{*}{Total} \\\cline{3-5}
 &  & 1 & 2 & 3 &  \\\hline
AltLex & Train & 611 & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} & 611 \\
 & Test & 416 & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} & 416 \\\hline
BECAUSE & Train & 1,185 & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} & 1,185 \\
 & Test & 60 & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} & 60 \\\hline
CTB & Train & 2,671 & 496 & 150 & 3,317 \\
 & Test & 372 & 82 & 38 & 492 \\\hline
ESL & Train & 6,447 & 5,873 & 5,094 & 17,414 \\
 & Test & 693 & 614 & 660 & 1,967 \\\hline
PDTB & Train & 22,598 & 18,671 & 1,190 & 42,459 \\
 & Test & 5,490 & 4,274 & 278 & 10,042 \\\hline
SemEval & Train & 8,000 & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} & 8,000 \\
 & Test & 2,717 & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} & 2,717 \\\hline
\multicolumn{2}{c|}{Total} & 51,260 & 30,010 & 7,410 & 88,680\\\hline
\end{tabular}
\caption{Sizes of train and test datasets by sentence length. We only retain examples with <=3 sentence length for our study.}\label{tab:split_data}
\end{table*}

==> tabs/UngroupData.tex <==
\begin{table*}[]
\centering
\begin{tabular}{l|l|l}\hline
Corpus & Split & Span \\\hline
AltLex & Train & 315 \\
 & Test & 127 \\\hline
BECAUSE & Train & 902 \\
 & Test & 46 \\\hline
PDTB & Train & 9,809 \\
 & Test & 2,294 \\\hline
\multicolumn{2}{c|}{Total} & 13,493\\\hline
\end{tabular}
\caption{Sizes of final train and test datasets available for Span Detection task. These numbers are the ungrouped version corresponding to the grouped ones in Table \ref{tab:final_data}.}\label{tab:ungrouped_data}
\end{table*}
